Hot phonon effects and suppressed Auger recombination on 3 $\mu$m room temperature lasing in HgTe-based multiple quantum well diodes

We propose an electrically pumped laser diode based on multiple HgTe quantum wells with band structure engineered for Auger recombination suppression. A model for accounting for hot phonons is developed for calculating the nonequilibrium temperature of electrons and holes. Using a comprehensive model accounting for carrier drift and diffusion, Auger recombination and hotphonon effects, we predict of lasing at $\lambda \sim 3 $ $\mu$m at room temperature in 2.2 nm HgTe/Cd$_{0.85}$Hg$_{0.15}$Te quantum well heterostructure. The output power in the pulse can reach up to 600 mW for 100 nanosecond-duration pulses.

==> table.tex <==
\begin{table*}[!t]
\caption{\label{tab:parameters}
Parameters of heterostructure layers: layer number (\#), thickness ($d$), composition, doping, electron ($\mu_n$) and hole ($\mu_p$) mobilities, bandgap ($E_g$)  and real part of the refractive index ($n'$) for the $\sim 3\,\mu$m wavelength. All the quantities are for 3D materials and temperature 300 K. In the graded-composition waveguide layers, the parameters vary linearly between their values in adjacent layers.}

%\begin{ruledtabular}
\begin{tabular}{*{8}c}
\hline
\hline
\# \& $d$  \& Composition \& Doping  \& $\mu_n$  \& $\mu_p$ \& $E_g$ \&   $n'$\cr
 \&  (nm) \&  \&  (cm$^{-3}$) \& ($\frac{\rm cm^2}{\rm V \cdot s}$) \& ($\frac{\rm cm^2}{\rm V \cdot s}$) \&  (eV)  \& \cr
 \hline
\multicolumn{8}{c}{Substrate}\\
1 \&  \& GaAs \& $n: 10^{18}$ \& 2361 \& 134 \& 1.42 \&  3.31 \cr \hline
\multicolumn{8}{c}{$n$-cladding layer}\\
2 \& 5000 \& CdTe \& $n: 10^{17}$ \& 111 \& 36 \& 1.49 \&   2.71\cr \hline
\multicolumn{8}{c}{$n$-waveguide layers}\\
\hline
3 \& 50 \& CdTe \& $n: 5\cdot 10^{17}$ \& 40 \& 16 \& 1.49 \& 2.7\cr 
4 \& 50 \& graded \cr 
5 \& 400 \& Cd$_{0.6}$Hg$_{0.4}$Te \& $n: 10^{17}$ \& 197 \& 36 \& 0.71   \& 2.86\cr
6 \& 50 \& graded \cr 
7 \& 30 \& Cd$_{0.9}$Hg$_{0.1}$Te \& $n:10^{18}$ \& 30 \& 11 \& 1.26  \& 2.74\cr
8 \& 10 \& graded \cr 
9 \& 10 \& Cd$_{0.85}$Hg$_{0.15}$Te \& $n:10^{16}$ \& 523 \& 73 \& 1.15  \& 2.78\cr
\hline
\multicolumn{8}{c}{active region}\\
10 \& 2.2 \& QW: HgTe \& 0 \& 523 \& 73 \& -0.14 \& 5.14\cr
11 \& 10 \& Cd$_{0.85}$Hg$_{0.15}$Te \& $n:10^{16}$ \& 523 \& 73 \& 1.15  \& 2.78\cr
\multicolumn{8}{c}{ + (5$\div$9) + 1/2 periods (2 layers in period)}\\
\hline
\multicolumn{8}{c}{$p$-waveguide layers}\\
12 \& 10 \& Cd$_{0.85}$Hg$_{0.15}$Te \& $n:10^{16}$ \& 523 \& 73 \& 1.15 \& 2.78\cr
13 \& 10 \& graded\cr
14 \& 20 \& CdTe \& $p: 5\cdot 10^{17}$ \& 40 \& 16 \& 1.49  \& 2.71\cr 
15 \& 30 \& CdTe \& $p: 1\cdot 10^{16}$ \& 414 \& 73 \& 1.49  \& 2.71\cr 
\hline
\multicolumn{8}{c}{$p$-cladding layer}\\
16 \& 3000 \& CdTe \& $p: 4\cdot 10^{16}$ \& 194 \& 51 \& 1.49  \& 2.71\cr 
\hline
\multicolumn{8}{c}{Au contact  layer}\\
\hline
\hline
\end{tabular}
%\end{ruledtabular}


\end{table*}
